An Analysis of Amazon Echo's Network Behavior

With over 20 million units sold since 2015, Amazon Echo, the Alexa-enabled smart speaker developed by Amazon, is probably one of the most widely deployed Internet of Things consumer devices. Despite the very large installed base, surprisingly little is known about the device's network behavior. We modify a first generation Echo device, decrypt its communication with Amazon cloud, and analyze the device pairing, Alexa Voice Service, and drop-in calling protocols. We also describe our methodology and the experimental setup. We find a minor shortcoming in the device pairing protocol and learn that drop-in calls are end-to-end encrypted and based on modern open standards. Overall, we find the Echo to be a well-designed device from the network communication perspective.

==> bibs/scripts/convert <==
#!/usr/bin/env bash

root=`pwd`
cache=$root/.cache
scripts=$root/scripts

#echo -n "## Deleting previously generated bib files..."
#find $root -name .orig -prune -or -name scripts -prune -or -name "*.bib" -exec rm {} \;
#find $root -name .orig -prune -or -name scripts -prune -or -empty -type d -delete
#echo "Done."

# Netbib from edas
#echo -n "## Processing Edas netbib..."
#rm -rf "$root/netbib"
#mkdir -p $root/netbib
#find $cache/netbib \
#  ! -name "i-d.bib" \
#  ! -name "rfc.bib" \
#  -name "*.bib" -exec cp {} $root/netbib \;
#echo "Done."

# Generate rfc.bib from rfc-index.xml
echo -n "## Processing RFC index..."
rm -f "$root/ietf/rfc.bib"
test -f $cache/ietf/rfc-index.xml && {
  mkdir -p $root/ietf
  xsltproc $scripts/rfc2bib.xsl $cache/ietf/rfc-index.xml | sed -E \
    -e 's/([_&%#$])/\\\1/g' \
    -e '/author=/s/([^ ]+[[:space:]]+(3rd|Jr\.))/{\1}/g' \
    -e "s/([^=])\"([^\"]*)\"/\1\`\`\2''/g" \
    -e "/author=/s/([^\"]),/\1 and /g" \
  > $root/ietf/rfc.bib
}
echo "Done."

#echo -n "## Processing I-Ds..."
#mkdir -p $root/ietf
#rm -f $root/ietf/i-d.bib
#tmp=`mktemp /tmp/idbib.XXXXXX`
#for f in $cache/ietf/bibxml3/*.xml ; do
#    $scripts/xmlrfc2bib $f > $tmp 2>/dev/null
#    if [ $? -ne 0 ] ; then
#        echo "Skipping broken" `basename $f`
#    else
#        cat $tmp >> $root/ietf/i-d.bib
#    fi
#done
#rm -rf "$tmp"
#echo "Done."


==> bibs/scripts/xmlrfc2bib <==
#!/bin/sh
magic='j2IrbfDl'
"""exec" python3.2 -E "$0" "$@" """#$magic"

if __name__ == '__main__':
    import sys
    if sys.argv[-1] == '#%s' % magic:
        del sys.argv[-1]
del magic

# TODO 
# * Find a way to fix documents with broken encoding before sending them
#   to the parser
# * Make sure all generated keys are unique, if not then make them unique
# * Generate place-holders for broken files
# * Switch to BeautifulSoup

import os
import re
import datetime
from lxml import etree

strings = {
    'wd'      : '{Working Draft}',
    'id'      : '{Internet-Draft}',
    'sec'     : '{IETF Secretariat}',
    'irfc'    : '{Internet Requests for Comments}',
    'rfc'     : '{RFC}',
    'ed'      : '{RFC Editor}',
    'wip'     : '{Work in Progress}',
    'id_url'  : 'http://tools.ietf.org/id/',
    'rfc_url' : 'http://www.rfc-editor.org/rfc/',
    'issn'    : '{2070-1721}'
}

month_abbrv = ['None', 'Jan', 'Feb', 'Mar', 'Apr', 'May', 'Jun', 'Jul', 'Aug',
               'Sep', 'Oct', 'Nov', 'Dec']

class ParseDone(Exception):
    """ This exception is used to stop the parsing of a document. It is raised
    after the parser has collected all the necessary information from the
    document.
    """

    def __init__(self):
        pass

class ParseError(Exception):
    """ This exception indicates a parse error, probably a badly formatted or
    corrupted RFC XML document.
    """

    def __init__(self, value):
        self.value = value

    def __str__(self):
        return repr(self.value)


def latex_escape(*text):
    """ Escape characters that have special meaning to LaTex. Return the
    escaped string.
    """
    res = []
    for t in text:
        res.append(re.sub('"([^"]*)"', "``\\1''", re.sub('([_&%#$])', '\\\\\\1', t)))
    if len(res) > 1:
        return tuple(res)
    else:
        return res[0]

def xml_normalize(*text):
    """ Remove leading and trailing white space and CR LF characters from
    strings retrieved from an XML document (attribute values or data). Return
    the normalized text.
    """
    res = []
    for t in text:
        res.append(re.sub('[\r\n \t]+', ' ', t).strip())
    if len(res) > 1:
        return tuple(res)
    else:
        return res[0]

def strip_end(text, suffix):
    """ Strip suffix from the end of text and return the shortened string.
    Raises an exception if text does not end with suffix.
    """
    if not text.endswith(suffix):
        raise Exception()
    return text[:-len(suffix)]

class RFC:
    def __init__(self, path):
        self.path = path
        self.filename = os.path.basename(path)
        self.reset()

    def reset(self):
        self.id = None
        self.number = None
        self.title = ''
        self.authors = []
        self.date = None
        self.state = []
        self.state.append("")

    def finish(self):
        """ After all values have been obtained from the XML document, fill in
        missing values and normalize all text obtained from XML.
        """
        # If the document didn't provide an ID then build one from the file
        # name
        if self.id is None \
                or self.id.strip() == '' \
                or self.id.strip() == 'DOCNAME'\
                or self.id.strip() == 'DRAFT;':
            name,ext = os.path.splitext(self.path)
            self.id = os.path.basename(name)
        self.id = xml_normalize(self.id)
        self.id = re.sub('[ \t]+', '-', self.id)

        # If the document did not provide a number then let's use the document
        # id as the number
        if self.number is None or self.id.strip() == '':
            self.number = self.id
        self.number = xml_normalize(self.number)

        # Normalize the document title
        self.title = xml_normalize(self.title)

    def parse(self):
        """ Parse the source XML document specified in constructor.
        """
        parser = etree.XMLParser(no_network = True, dtd_validation = False,
                                 load_dtd = False, recover = True,
                                 resolve_entities = True, target = self)

        try:
            etree.parse(self.path, parser)    
        except ParseDone:
            self.finish()
            return
        raise ParseError("Malformed XML RFC document")

    def get_date(self):
        """ Obtain the document date. First try to obtain it from the
        document's date element and then fill the missing elements from the
        file's modification date.
        """
        d = datetime.datetime.fromtimestamp(os.path.getmtime(self.path))
        year = d.year
        month = month_abbrv[d.month]
        day = d.day
        if self.date is None:
            return
        try:
            year = self.date['year']
        except KeyError:
            pass
        try:
            month = self.date['month'].strip()[0:3].capitalize()
        except KeyError:
            pass
        try:
            day = self.date['day']
        except KeyError:
            pass
        return year,month,day

    def get_author_list(self):
        """ Compile the BibTeX author list from the list of authors obtained
        from the XML document.
        """
        res = ''
        for i in range(len(self.authors)):
            try:
                # First try to see if we can build a name of the form "Last, First"
                name = xml_normalize(self.authors[i]['surname']) + ", "
                name += strip_end(xml_normalize(self.authors[i]['fullname']),
                                  xml_normalize(self.authors[i]['surname'])).strip()
            except:
                # Next try "Last, Initials"
                try:
                    name = xml_normalize(self.authors[i]['surname']) + ", "
                    name += xml_normalize(self.authors[i]['initials'])
                except:
                    # Finally, try to use just the fullname, i.e., "First Last"
                    try:
                        name = xml_normalize(self.authors[i]['fullname'])
                    except:
                        # If none of the above worked, put a placeholder into
                        # the author list
                        name = '{}'

            res += name
            if i < len(self.authors) - 1:
                res += ' and '
        return res

    def get_bibtex(self):
        """ Put together the BibTex entry for the document and return it as
        text.
        """
        b = ''

        b += '@techreport{{{},\n'.format(latex_escape(self.id))
        b += '  author="{}",\n'.format(self.get_author_list())
        b += '  title="{{{}}}",\n'.format(latex_escape(self.title))
        b += '  howpublished="{}",\n'.format(latex_escape(strings['wd']))
        b += '  type="{}",\n'.format(latex_escape(strings['id']))
        b += '  number="{}",\n'.format(latex_escape(self.number))
        year, month, day = self.get_date()
        b += '  year={},\n  month={},\n  day={},\n'.format(
            year,latex_escape(month), day)
        b += '  institution="{}",\n'.format(latex_escape(strings['sec']))
        name,ext = os.path.splitext(self.path)
        b += '  url={{{}}},\n'.format(latex_escape(strings['id_url'] +
                                                   os.path.basename(name)))
        b += '}\n'
        return b

    def start(self, tag, attrib):
        """ This method received start-of-element SAX parser events. It keeps
        track of the current position in the document and extracts pieces
        needed to generate the BibTex entry.
        """
        if self.state[-1] == "":
            if tag == "rfc":
                try:
                    name = attrib['docName']
                    self.id = name
                except KeyError:
                    pass
                self.state.append(tag)
            else:
                raise ParseError("Top-level element is not <rfc>: " + tag)
        elif self.state[-1] == "rfc":
            if tag == "front":
                self.state.append(tag)
            else:
                self.state.append("other")
        elif self.state[-1] == "front":
            if tag == "author":
                self.state.append(tag)
                self.authors.append(attrib)
            elif tag == "title":
                self.state.append(tag)
            elif tag == "date":
                self.state.append(tag)
                self.date = attrib
            else:
                self.state.append("other")
        else:
            self.state.append("other")

    def end(self, tag):
        """ This method is the receiver for end-of-tag SAX events generated by
        the parser. It stops parsing by raising ParseDone exception when
        </front> is reached.
        """
        self.state.pop()
        if tag == "front":
            raise ParseDone()

    def data(self, data):
        """ This method receives data SAX events. It is currently used to
        extract the document title text.
        """
        if self.state[-1] == "title":
            self.title += data

    def close(self):
        pass


rfc = RFC(sys.argv[1])
rfc.parse()
print(rfc.get_bibtex())

